Pseudo Flow Consistency for Self-Supervised 6D Object Pose Estimation

Most self-supervised 6D object pose estimation methods can only work with additional depth information or rely on the accurate annotation of 2D segmentation masks, limiting their application range. In this paper, we propose a 6D object pose estimation method that can be trained with pure RGB images without any auxiliary information. We first obtain a rough pose initialization from networks trained on synthetic images rendered from the target's 3D mesh. Then, we introduce a refinement strategy leveraging the geometry constraint in synthetic-to-real image pairs from multiple different views. We formulate this geometry constraint as pixel-level flow consistency between the training images with dynamically generated pseudo labels. We evaluate our method on three challenging datasets and demonstrate that it outperforms state-of-the-art self-supervised methods significantly, with neither 2D annotations nor additional depth images.

==> tables/ablate_hyper_param.tex <==
% \begin{tabular}{c|ccccc|cccc|c|cccc}
%     \toprule
%     $M$     & MSPD          & MSSD          & VSD           & Avg.      $N$     & MSPD          & MSSD          & VSD           & Avg.          & $\tau$        & MSPD      & MSSD      & VSD       & Avg. \\
%     \midrule
%     2       &               &               &               &2       &               &               &               &               & 0.5           &  0.776        & 0.741         & 0.655         & 0.724\\
%     3       & 0.779         & 0.747         & 0.667         & 0.731         & {\bf 1.}      & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733}\\
%     {\bf 4} & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733}   & 4.            & 0.777         & 0.748         & 0.662         & 0.729\\
%     5       & 0.782         & 0.738         & 0.653         & 0.725         & 8.            & 0.772         & 0.736         & 0.654         & 0.721\\
%     6       & 0.780         & 0.733         & 0.649         & 0.721         & 16.           & 0.769         & 0.734         & 0.647         & 0.717\\
%     \bottomrule
% \end{tabular}

% \begin{tabular}{c|ccccc|c|ccccc|c|ccccc}
%     \toprule
%     $M$     & MSPD      & MSSD      & VSD       & Avg.      & $N$       & MSPD          & MSSD          & VSD           & Avg.          & $\tau$        & MSPD      & MSSD      & VSD       & Avg. \\
%     \midrule
%     1       &           &           &           &           & 1         & 0.776         & 0.728        & 0.645        & 0.716         & 0.5           &  0.776        & 0.741         & 0.655         & 0.724\\
%     {\bf 2} &{\bf 0.785}&{\bf 0.749}&{\bf 0.664}&{\bf 0.733}& 2         & 0.779         & 0.747         & 0.667         & 0.731         & {\bf 1.}      & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733}\\
%     3       &           &           &           &           &{\bf 3}    & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733}   & 4.            & 0.777         & 0.748         & 0.662         & 0.729\\
%     4       &           &           &           &           &4          & 0.782         & 0.738         & 0.653         & 0.725         & 8.            & 0.772         & 0.736         & 0.654         & 0.721\\
%     5       &           &           &           &           &5          & 0.780         & 0.733         & 0.649         & 0.721         & 16.           & 0.769         & 0.734         & 0.647         & 0.717\\
%     \bottomrule
% \end{tabular}

% \begin{tabular}{c|ccccc|c|ccccc|c|ccccc}
%    \toprule
%    $M$     & MSPD      & MSSD      & VSD       & Avg.      &ADD    & $N$       & MSPD          & MSSD          & VSD           & Avg.          & ADD      & $\tau$        & MSPD           & MSSD         & VSD          & Avg.         & ADD\\
%    \midrule
%    1       &           &           &           &           &      & 1         & 0.776         & 0.728         & 0.645         & 0.716         &          & 0.5           &  0.776        & 0.741         & 0.655         & 0.724       &  \\
%    {\bf 2} &{\bf 0.785}&{\bf 0.749}&{\bf 0.664}&{\bf 0.733}&      & 2         & 0.779         & 0.747         & 0.667         & 0.731         &          & {\bf 1.}      & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733} &  \\
%    3       &           &           &           &           &      &{\bf 3}    & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733}   &          & 4.            & 0.777         & 0.748         & 0.662         & 0.729       &  \\
%    4       &           &           &           &           &      &4          & 0.782         & 0.738         & 0.653         & 0.725         &          & 8.            & 0.772         & 0.736         & 0.654         & 0.721       &  \\
%    5       &           &           &           &           &      &5          & 0.780         & 0.733         & 0.649         & 0.721         &          & 16.           & 0.769         & 0.734         & 0.647         & 0.717       &  \\
%    \bottomrule
% \end{tabular}

% \begin{tabular}{c|ccccc}
%    \toprule
%             & MSPD      & MSSD      & VSD       & Avg.      &ADD \\
%    \midrule
%    \multicolumn{6}{c}{\textit{Number of Views for photometric consistency $M$}} \\
%    \midrule
%    1        &  0.780          &0.745            & 0.662           & 0.729        & 66.8     \\
%    {\bf 2}  &{\bf 0.785}      &{\bf 0.749}      &{\bf 0.664}      &{\bf 0.733}   & 67.4      \\
%    3        & 0.782           & 0.752           & 0.661           & 0.731        & {\bf 67.6}     \\
%    4        & 0.774           & 0.741           & 0.657           & 0.724        & 66.8         \\
%    5        & 0.772           & 0.736           & 0.648           & 0.719        & 65.2        \\
%    \midrule
%    \multicolumn{6}{c}{\textit{Number of Views for geometry consistency $N$}} \\
%    \midrule
%    1        & 0.776           & 0.728           & 0.645           & 0.716         & 61.6      \\
%    2        & 0.779           & 0.747           & 0.667           & 0.731         & 67.0   \\
%    {\bf 3}  & {\bf 0.785}     & {\bf 0.749}     & {\bf 0.664}     & {\bf 0.733}   & {\bf 67.4}   \\
%    4        & 0.782           & 0.738           & 0.653           & 0.725         & 64.7    \\
%    5        & 0.780           & 0.733           & 0.649           & 0.721         & 63.3    \\
%    \midrule
%    \multicolumn{6}{c}{\textit{Variance threshold $\tau$}} \\
%    \midrule
%    0.5           &  0.776        & 0.741         & 0.655         & 0.724       & 65.0        \\
%    {\bf 1.}      & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733} & 67.4         \\
%    4.            & 0.777         & 0.748         & 0.662         & 0.729       & {\bf 67.6}         \\
%    8.            & 0.772         & 0.736         & 0.654         & 0.721       & 65.4 \\
%    16.           & 0.769         & 0.734         & 0.647         & 0.717       & 64.6\\
%    \bottomrule
% \end{tabular}


\begin{tabular}{cc|cccc}
   \toprule
                        &           & MSPD          & MSSD          & VSD       &ADD \\
   \midrule
   % \multicolumn{5}{c}{\textit{Number of Views for photometric consistency $m$}} \\
                        &2          &  0.780          &0.745            & 0.662           & 66.8     \\
                        &{3}        &{\bf 0.785}      &{\bf 0.749}      &{\bf 0.664}      & 67.4      \\
    $m$                 &4          & 0.782           & 0.752           & 0.661           & {\bf 67.6}     \\
                        &5          & 0.774           & 0.741           & 0.657           & 66.8         \\
                        &6          & 0.772           & 0.736           & 0.648           & 65.2        \\
   \midrule
   % % \multicolumn{5}{c}{\textit{Number of Views for geometry consistency $n$}} \\
   % % \midrule
   &2        & 0.776           & 0.728           & 0.645           & 61.6      \\
   &3        & 0.779           & 0.747           & 0.667           & 67.0   \\
   $n$&{4}  & {\bf 0.785}     & {\bf 0.749}     & {\bf 0.664}     & {\bf 67.4}   \\
   &5        & 0.782           & 0.738           & 0.653           & 64.7    \\
   &6        & 0.780           & 0.733           & 0.649           & 63.3    \\
   % \midrule
   % % \multicolumn{5}{c}{\textit{Variance threshold $\tau$}} \\
   \midrule
   &0.5           &  0.776        & 0.741         & 0.655         & 65.0        \\
   &{1.}      & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & 67.4         \\
   $\tau$&4.            & 0.777         & 0.748         & 0.662         & {\bf 67.6}         \\
   &8.            & 0.772         & 0.736         & 0.654         & 65.4 \\
   &16.           & 0.769         & 0.734         & 0.647         & 64.6\\
   \bottomrule
\end{tabular}

==> tables/ablate_lmo.tex <==
% \begin{tabular}{l|ccccc}
%     \toprule
%     Method              & MSPD      & MSSD      & VSD       & Avg.      & ADD \\
%     \midrule
%     WDR-Pose*           & 0.748     & 0.484     & 0.367     & 0.533     & 35.8          \\
%     +RAFT-LB            & 0.871     & 0.677     & 0.532     & 0.693     & 57.0       \\
%     +RAFT-UB            &{\bf 0.876}&{\bf 0.746}&{\bf 0.587}&{\bf 0.736}& {\bf 66.8}       \\
%     {\bf+RAFT(Ours)}    & 0.859     & 0.725     & 0.574     & 0.719     & 65.3      \\
%      \bottomrule
% \end{tabular}


\begin{tabular}{l|cccc}
    \toprule
    Method                  & MSPD      & MSSD      & VSD                   & ADD \\
    \midrule
    Initialization          & 0.748                 & 0.484                 & 0.367     & 35.8          \\
    + Ours (Synthetic)        &\underline{0.871}      & 0.677                 & 0.532     & 57.0       \\
    + Ours (Real)          &{\bf 0.876}            &{\bf 0.746}            &{\bf 0.587}&{\bf 66.8}       \\
    + Ours (SSL)              & 0.859                 & \underline{0.725}     & \underline{0.574} & \underline{65.4}      \\
     \bottomrule
\end{tabular}

==> tables/compare_bop.tex <==
% \begin{tabular}{c|cccc}
%     \toprule
%     Method      & MSPD          & MSSD          & VSD       & Avg. \\
%     \midrule
%     \multicolumn{5}{c}{\textit{YCB-V}}\\
%     \midrule
%     {\bf Ours}  & {\bf 0.775}   & {\bf 0.740}   & {\bf 0.656}   & {\bf 0.723} \\
%     Ours-LB     & {\bf 0.775}   & {\bf 0.740}   & {\bf 0.656}   & {\bf 0.723} \\
%     Ours-UB     & {\bf 0.775}   & {\bf 0.740}   & {\bf 0.656}   & {\bf 0.723} \\
%     SurfEmb     & 0.773         & 0.620         & 0.548         & 0.647 \\
%     CosyPose    & 0.653         & 0.554         & 0.516         & 0.574 \\
%     EPOS        & 0.621         & 0.464         & 0.411         & 0.499 \\
%     CDPNv2      & 0.511         & 0.399         & 0.260         & 0.390 \\
%     \midrule
%     \multicolumn{5}{c}{\textit{LM-O}}\\
%     \midrule
%     {\bf Ours}  & {\bf 0.859}   & {\bf 0.725}   & {\bf 0.574}   & {\bf 0.719} \\
%     Ours-LB     & {\bf 0.775}   & {\bf 0.740}   & {\bf 0.656}   & {\bf 0.723} \\
%     Ours-UB     & {\bf 0.775}   & {\bf 0.740}   & {\bf 0.656}   & {\bf 0.723} \\
%     CIR         & 0.831         & 0.633         & 0.501         & 0.655 \\
%     SurfEmb     & 0.851         & 0.640         & 0.497         & 0.647 \\
%     CosyPose    & 0.812         & 0.606         & 0.480         & 0.633 \\
%     CDPNv2      & 0.815         & 0.612         & 0.445         & 0.612 \\
%     \bottomrule
% \end{tabular}

\begin{tabular}{ll|cccc|cccc}
    \toprule
    \multirow{2}{*}{Method}             & \multirow{2}{*}{Supervison}& \multicolumn{4}{c|}{LM-O}                                     & \multicolumn{4}{c}{YCB-V} \\
    ~                                   & ~         & MSPD      & MSSD      & VSD       & Avg.                      & MSPD      & MSSD      & VSD       & Avg.      \\
    \midrule
    CDPNv2~\cite{CDPN_2019_iccv}        & Syn       & 0.815         & 0.612         & 0.445         & 0.612         & 0.511         & 0.399         & 0.260         & 0.390 \\
    EPOS~\cite{hodan2020epos}           & Syn       & 0.659         & 0.380         & 0.290         & 0.443         & 0.621         & 0.464         & 0.411         & 0.499 \\
    Cosypose~\cite{cosypose_2020_eccv}  & Syn       & 0.812         & 0.606         & 0.480         & 0.633         & 0.653         & 0.554         & 0.516         & 0.574 \\
    SurfEmb~\cite{surfemb_2022_cvpr}    & Syn       & 0.851         & 0.640         & 0.497         & 0.647         & 0.773         & 0.620         & 0.548         & 0.647 \\
    CIR~\cite{coupled_2022_cvpr}        & Syn       & 0.831         & 0.633         & 0.501         & 0.655         & -              & -             & -             & -     \\
    NCF~\cite{huang2022neural}          & Syn       & -             &  -            & -             & 0.632         & -             & -             & -             & 0.673 \\
    \midrule
    Ours-LB                             & Syn       & 0.871         & 0.677         & 0.532         & 0.693         & 0.761         & 0.605         & 0.534         & 0.633 \\
    Ours-UB                             & Syn+Real  & 0.876         & 0.746         & 0.587         & 0.736         & 0.803         & 0.752         & 0.686         & 0.747  \\
    {\bf Ours}                          & Syn+Self & {\bf 0.859}   & {\bf 0.725}   & {\bf 0.574}   & {\bf 0.719}    & {\bf 0.785}   & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733} \\
    \bottomrule
\end{tabular}

==> tables/compare_lm_lmo.tex <==
\begin{tabular}{c|cccc|ccccc}
    \toprule
    Supervision     & \multicolumn{4}{c|}{Synthetic}                     & \multicolumn{4}{c}{Synthetic + Real(w/o annotation)}      \\
    \midrule
    Dataset         & AAE        & MHP       & DPODv2    & DeepIM*      & DSC      & Sock et al.   & Self6D    & Self6D++    & {\bf Ours}  \\
    \midrule
    LM             &  31.4      & 38.8      & 81.2       & 88.0         & 58.6      & 60.6          & 58.9      & 85.6      & 92.1\\
    LM-O           & -          & -         &  -         & 62.5         & 24.8          & 22.8          & 32.1      & 59.8      & 64.8\\
    \bottomrule
    
\end{tabular}

==> tables/compare_ssl.tex <==
% \begin{tabular}{cc|ccccc}
%     \toprule
%     Geo.            & Photo.                 &  MSPD        & MSSD          & VSD           & Avg.        & ADD\\
%     \midrule
%      \multicolumn{7}{c}{\textit{EMA Teacher}} \\
%      \midrule
%      -              & -                     &  0.759        &  0.589        & 0.519         & 0.622      & 30.9 \\
%       -             & \cmark                &  0.765        &  0.631        & 0.578         & 0.658       & 37.5          \\
%     \cmark          & -                     &  0.780        &  0.711        & 0.658         & 0.716       & 64.2   \\
%     \cmark          & \cmark                &  {\bf 0.785}  & {\bf 0.749}   & {\bf 0.664}   & {\bf 0.733}  & {\bf 67.4}\\
%     \midrule
%     \multicolumn{7}{c}{\textit{Fixed Teacher}} \\
%     \midrule
%      -              & -                     &  0.764        & 0.590         &  0.522        & 0.625   & 31.4\\
%      -               & \cmark               &  0.765        & 0.594        &  0.519         & 0.626    & 31.9 \\
%     \cmark          & -                     &  0.770        & 0.610         &  0.534        & 0.638   & 35.7 \\
%     \cmark          & \cmark                &  {\bf 0.774}  & {\bf 0.623}   & {\bf 0.553}   & {\bf 0.650}   & {\bf 36.8}\\
%     \midrule
%     \multicolumn{7}{c}{\textit{Identity Teacher}} \\
%     \midrule
%      -              & -                     & \multicolumn{5}{c}{divergence}       \\
%       -             & \cmark                & \multicolumn{5}{c}{divergence} \\
%     \cmark          & -                     & 0.778        & 0.652         & 0.562          & 0.664        & 41.7\\
%     \cmark          & \cmark                & {\bf 0.780}  & {\bf 0.674}   & {\bf 0.591}    & {\bf 0.682}  & {\bf 46.5} \\
%     \midrule
%     \multicolumn{7}{c}{\textit{Unsupervised Loss}} \\
%     \midrule
%     -              & -                     &  0.751        & 0.565         & 0.488          &  0.601   & 28.7\\
%     \bottomrule
% \end{tabular}


% \begin{tabular}{cc|cccc}
%    \toprule
%    $\mathcal{L}_{flow}$ & $\mathcal{L}_{photo}$                 &  MSPD        & MSSD          & VSD                   & ADD\\
%    \midrule
%     \multicolumn{6}{c}{\textit{EMA Teacher}} \\
%     \midrule
%     -              & -                     &  0.759        &  0.589        & 0.519         & 30.9 \\
%      -             & \cmark                &  0.765        &  0.631        & 0.578          & 37.5          \\
%    \cmark          & -                     &  0.780        &  0.711        & 0.658          & 64.2   \\
%    \cmark          & \cmark                &  {\bf 0.785}  & {\bf 0.749}   & {\bf 0.664}     & {\bf 67.4}\\
%    \midrule
%    \multicolumn{6}{c}{\textit{Fixed Teacher}} \\
%    \midrule
%     -              & -                     &  0.764        & 0.590         &  0.522        & 31.4\\
%     -               & \cmark               &  0.765        & 0.594        &  0.519         & 31.9 \\
%    \cmark          & -                     &  0.770        & 0.610         &  0.534        & 35.7 \\
%    \cmark          & \cmark                &  {\bf 0.774}  & {\bf 0.623}   & {\bf 0.553}   & {\bf 36.8}\\
%    \midrule
%    \multicolumn{6}{c}{\textit{Identity Teacher}} \\
%    \midrule
%     -              & -                     & \multicolumn{4}{c}{divergence}       \\
%      -             & \cmark                & \multicolumn{4}{c}{divergence} \\
%    \cmark          & -                     & 0.778        & 0.652         & 0.562           & 41.7\\
%    \cmark          & \cmark                & {\bf 0.780}  & {\bf 0.674}   & {\bf 0.591}      & {\bf 46.5} \\
%    \midrule
%    \multicolumn{6}{c}{\textit{Unsupervised Loss}} \\
%    \midrule
%    -              & -                     &  0.751        & 0.565         & 0.488            & 28.7\\
%    \bottomrule
% \end{tabular}


\begin{tabular}{cc|cccc|cc|cccc|cc|cccc}
  \toprule
  $\mathcal{L}_{flow}$ & $\mathcal{L}_{photo}$ &  MSPD  & MSSD  & VSD & ADD 
  &$\mathcal{L}_{flow}$ & $\mathcal{L}_{photo}$ &  MSPD  & MSSD  & VSD & ADD
  &$\mathcal{L}_{flow}$ & $\mathcal{L}_{photo}$ &  MSPD  & MSSD  & VSD & ADD \\
  \midrule
  \multicolumn{6}{c|}{\textit{EMA Teacher}} & \multicolumn{6}{c|}{\textit{Fixed Teacher}} &  \multicolumn{6}{c}{\textit{Identity Teacher}}  \\
  \midrule
  
  -              & -                     &  0.759        &  0.589        & 0.519         & 30.9 &
  -              & -                     &  0.764        & 0.590         &  0.522        & 31.4&
  -              & -                     & \multicolumn{4}{c}{divergence}       \\

  -               & \cmark               &  0.765        & 0.594        &  0.519         & 31.9 &
    -             & \cmark                &  0.765        &  0.631        & 0.578          & 37.5   &
    -             & \cmark                & \multicolumn{4}{c}{divergence} \\

  \cmark          & -                     &  0.780        &  0.711        & 0.658          & 64.2   &
  \cmark          & -                     &  0.770        & 0.610         &  0.534        & 35.7 &
  \cmark          & -                     & 0.778        & 0.652         & 0.562           & 41.7\\

  \cmark          & \cmark                &  {\bf 0.785}  & {\bf 0.749}   & {\bf 0.664}     & {\bf 67.4}&
  \cmark          & \cmark                &  {\bf 0.774}  & {\bf 0.623}   & {\bf 0.553}   & {\bf 36.8}&
  \cmark          & \cmark                & {\bf 0.780}  & {\bf 0.674}   & {\bf 0.591}      & {\bf 46.5} \\

  \bottomrule
  % \midrule
  % -              & -                     &  0.751        & 0.565         & 0.488            & 28.7\\
  % \bottomrule
\end{tabular}

==> tables/compare_tless.tex <==
% \begin{tabular}{l|cccc}
%     \toprule
%     Method              & MSPD      & MSSD      & VSD       & Avg.     \\
%     \midrule
%     DPODv2              & 0.595     & 0.491     & 0.469     & 0.518     \\
%     CIR                 & 0.798     & 0.684     & \underline{0.663}     & 0.715     \\ 
%     CosyPose            & 0.821     &{\bf 0.695}&{\bf 0.669}& {\bf 0.728}    \\
%     \midrule
%     Initialization      & 0.787     & 0.514     & 0.464     & 0.588    \\
%     Ours + Synthetic    & 0.826     & 0.666     & 0.627     & 0.707    \\
%     Ours + Mixed        &{\bf 0.831}& \underline{0.691}& 0.649     & \underline{0.723}     \\
%     {\bf Ours + SSL}    &\underline{0.828}& 0.687& 0.639     & 0.718     \\
%     \bottomrule
% \end{tabular}


\begin{tabular}{llcccc}
    \toprule
    Method                  & MSPD              & MSSD              & VSD               & ADD(-S)     \\
    \midrule
    Initialization      & 0.787             & 0.514             & 0.464             & 65.1          \\
    + Ours (Synthetic)  & 0.826             & 0.666             & 0.627             & 75.0           \\
    + Ours (Real)        &{\bf 0.831}        &\textbf{0.691}  & \textbf{0.649}      & {\bf 80.6}           \\
    {\bf + Our (SSL)}    &\underline{0.828}  & \underline{0.687}  & \underline{0.639} & \underline{78.2}      \\
    % \midrule
    % DPODv2              & 0.595             & 0.491             & 0.469             & - \\
    % CIR            & 0.798             & 0.684             & \textbf{0.663} & -         \\ 
    % CosyPose            & 0.821             &{\bf 0.695}        &{\bf 0.669}        & -          \\
    \bottomrule
\end{tabular}

==> tables/compare_unsup.tex <==
\begin{tabular}{ccccc}
    \toprule
    Method          & MSPD      & MSSD      & VSD       & Avg.   \\
    \midrule
    Unsupervise Loss    &       &           &           &       \\
    Ours            &           &           &           &       \\
    \bottomrule
\end{tabular}

==> tables/compare_ycbv.tex <==
% \begin{tabular}{cccccc}
%     \toprule
%      % Method         & SO-Pose       & RePose        & RNNPose     & Self6D++      & {\bf Ours} \\
%      % \midrule   
%      % AUC            & {\bf 83.9}    & 80.8          & \underline{83.1}    & 78.9          & 82.6\\
%      % ADD-0.1d       & 56.8          & 63.3          & \underline{66.4}          & -             & {\bf 67.7}\\
%      \bottomrule
% \end{tabular}

\begin{tabular}{cccccc}
    \toprule
     
                    & MSPD          & MSSD              & VSD               & ADD(-S)           & AUC \\
     \midrule
     Self6D++       & -             & -                 & -                 & -             & 80.0\\
     {\bf Ours}     & {0.785}   &{0.749}        & {0.664}       & {67.7}    & {\bf 82.6}\\
     \bottomrule
\end{tabular}



==> tables/dataratio.tex <==
% \begin{tabular}{c|ccccccccc}
%     \toprule
%     Ratio(\%)      & 0          & 1         & 5             & 10            & 20        & 40            & 80        & 100 \\
%     \midrule
%     MSPD           & 0.761      & 0.778    &  0.782        & 0.784         & 0.782      & 0.780         & 0.783          & {\bf 0.785}         \\
%     MSSD           & 0.605      & 0.743    &  0.744        & 0.745         & 0.748      & {\bf 0.752}   & 0.750          & 0.749          \\
%     VSD            & 0.534      & 0.661    &  0.663        & 0.664         & {\bf 0.665}& 0.664         & 0.660         & 0.664     \\
%     % Avg.           & 0.633      & 0.727          &  0.729        & 0.731        & 0.732      & 0.732         & 0.731      & {\bf 0.733}     \\
%     ADD            & 41.7       & 61.9      &  63.2        & 65.5         & 65.8       & 66.8          & 67.0        & {\bf 67.4}          \\
%     \bottomrule
% \end{tabular}


\begin{tabular}{ccccc}
    \toprule
     Ratio  & MSPD      & MSSD          & VSD       & ADD \\
     \midrule
     0      & 0.761     & 0.605         & 0.534     & 41.7  \\
     1      & 0.778     & 0.743         & 0.661    & 61.9       \\
     5      & 0.782    &  0.744        &  0.663    &   63.2\\
     10     & 0.784     & 0.745         & 0.664     & 65.5 \\
     20     & 0.782     &  0.748        & 0.665         & 65.8\\
     40     & 0.780     & 0.749         & 0.664     & 66.8 \\
     80     & 0.783     & 0.748         & 0.660     & 67.0 \\
     100    & {\bf 0.785}& {\bf 0.749}      & {\bf 0.665}     & {\bf 67.4}\\
     \bottomrule
\end{tabular}

==> tables/training_seq_num.tex <==
\begin{tabular}{c|c}
     &  \\
     & 
\end{tabular}
